Junta correlation is testable

The problem of tolerant junta testing is a natural and challenging problem which asks if the property of a function having some specified correlation with a $k$-Junta is testable. In this paper we give an affirmative answer to this question: We show that given distance parameters $\frac{1}{2} >c_u>c_{\ell} \ge 0$, there is a tester which given oracle access to $f:\{-1,1\}^n \rightarrow \{-1,1\}$, with query complexity $ 2^k \cdot \mathsf{poly}(k,1/|c_u-c_{\ell}|)$ and distinguishes between the following cases: $\mathbf{1.}$ The distance of $f$ from any $k$-junta is at least $c_u$; $\mathbf{2.}$ There is a $k$-junta $g$ which has distance at most $c_\ell$ from $f$. This is the first non-trivial tester (i.e., query complexity is independent of $n$) which works for all $1/2 > c_u > c_\ell \ge 0$. The best previously known results by Blais \emph{et~ al.}, required $c_u \ge 16 c_\ell$. In fact, with the same query complexity, we accomplish the stronger goal of identifying the most correlated $k$-junta, up to permutations of the coordinates. We can further improve the query complexity to $\mathsf{poly}(k, 1/|c_u-c_{\ell}|)$ for the (weaker) task of distinguishing between the following cases: $\mathbf{1.}$ The distance of $f$ from any $k'$-junta is at least $c_u$. $\mathbf{2.}$ There is a $k$-junta $g$ which is at a distance at most $c_\ell$ from $f$. Here $k'=O(k^2/|c_u-c_\ell|)$. Our main tools are Fourier analysis based algorithms that simulate oracle access to influential coordinates of functions.

==> Markov.tex <==
\section{Markov chains and random walks}~\label{sec:Markov}
We begin by recalling some basic terminology regarding Markov chains. 

We will  need a ``Chernoff-type" bound for Markov chains. Several such formulations are known~(e.g.,~\cite{gillman1998chernoff, healy2008randomness, GLSS18} which have many applications in computer science (see the survey~\cite{vadhan2012pseudorandomness}). In particular, we will need the following bound due to 

We now apply this theorem to the Markov chain defined by the Bonami-Beckner noise operator. In particular, let us say $y \sim T_{\rho}(x)$ if $y = x \oplus z$ and $z \sim \mathbf{Z}_{\eta}$ where all the coordinates of $\eta$ is $\rho$. 
\begin{lemma}~\label{lem:bias}
For any $\rho \in [-1,1]$, let us define the Markov chain $\mathcal{M}_\rho$  by the sequence $(\mathbf{x}_i)_{i=1}^\infty$ where $\mathbf{x}_{i+1} \sim T_{\rho}(\mathbf{x}_i)$. Let $f: \{-1,1\}^n \rightarrow [-1,1]$   and let $\gamma>0$. Further, let $\mathbf{x}_1 \sim \{-1,1\}^n$. Then, for any $T \ge \frac{C \log (1/\delta)}{\gamma^2 \cdot (1-\rho)}$ where $C$ is sufficiently large,
\[
\Pr\bigg[ \bigg| \frac{f(\mathbf{x}_1) + \ldots + f (\mathbf{x}_T)}{T}  - \mathbf{E}_{x \sim \{-1,1\}^n} [f(x)]\bigg| > \gamma \bigg] \leq \delta. 
\] 
\end{lemma}
\begin{proof}
First of all, observe that the Markov chain $\mathcal{M}_\rho$ is irreducible and ergodic. Further, the stationary distribution $\boldsymbol{\pi}$ is uniform on the hypercube -- which is identical to the distribution of $\mathbf{x}_1$. Let us now apply Theorem~\ref{thm:Chernoff-expander} to the Markov chain $\mathcal{M}_\rho$ and the function $$g(x) = \frac{f(x) - \mathbf{E}_{z \in \{-1,1\}^n} [f(z)]}{2}$$. Then, we get the stated claim. 
\end{proof}

